Group-Evolving Agents: Open-Ended Self-Improvement via Experience Sharing

Open-ended self-improving agents can autonomously modify their own structural designs to advance their capabilities and overcome the limits of pre-defined architectures, thus reducing reliance on human intervention. We introduce Group-Evolving Agents (GEA), a new paradigm for open-ended self-improvements, which treats a group of agents as the fundamental evolutionary unit, enabling explicit experience sharing and reuse within the group throughout evolution. Unlike existing open-ended self-evolving paradigms that adopt tree-structured evolution, GEA overcomes the limitation of inefficient utilization of exploratory diversity caused by isolated evolutionary branches. We evaluate GEA on challenging coding benchmarks, where it significantly outperforms state-of-the-art self-evolving methods (71.0% vs. 56.7% on SWE-bench Verified, 88.3% vs. 68.3% on Polyglot) and matches or exceeds top human-designed agent frameworks (71.8% and 52.0% on two benchmarks, respectively). Analysis reveals that GEA more effectively converts early-stage exploratory diversity into sustained, long-term progress, achieving stronger performance under the same number of evolved agents. Furthermore, GEA exhibits consistent transferability across different coding models and greater robustness, fixing framework-level bugs in 1.4 iterations on average, versus 5 for self-evolving methods.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec_arxiv/main_table.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of different reasoning methods and DMLR across various benchmarks. All metrics are reported in Accuracy (\%).
Results are evaluated over a diverse suite of mathematics reasoning, visual reasoning, and multimodal composition tasks under multiple backbone models.}

\large
\renewcommand{\arraystretch}{1.05}
\resizebox{0.9\linewidth}{!}{%
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll@{\hspace{6pt}}ccc@{\hspace{6pt}}cc@{\hspace{6pt}}cc}
\toprule[1.5pt]
\multicolumn{2}{c}{} &
\multicolumn{3}{c}{\textbf{Mathematics Reasoning $\uparrow$}} &
\multicolumn{2}{c}{\textbf{Visual Reasoning $\uparrow$}} &
\multicolumn{2}{c}{\textbf{Multimodal Composition $\uparrow$}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\textbf{Method} & \textbf{Model} &
$\mathrm{MathVista}_{\text{mini}}$ &
$\mathrm{MathVision}_{\text{mini}}$ &
MM-Math &
HallusionBench &
MMVP & MMStar &
ScienceQA \\
\midrule

Vanilla &  & 58.7 & 21.6 & 37.5 & 65.4 & 68.7 & 59.3 & 49.7 \\
Multimodal COT &  & 56.4 & 21.8 & 35.6 & 63.6 & 68.1 & 57.9 & 49.5  \\
CCOT &  & 57.8 & 22.5 & 36.3 & 64.9 & 69.0 & 58.7 & 50.2 \\
ICoT &  & 58.9 & 23.3 & 37.0 & 65.5 & 69.3 & 60.4 & 50.4\\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-5}{*}[1pt]{\rotatebox{90}{\parbox{2.5cm}{\centering \fontsize{11pt}{13pt}\selectfont Qwen2.5 \\ VL 7B}}}
 & \textbf{59.1} \up{0.40\%} & \textbf{24.4} \up{2.8\%} & 38.8 \up{1.3\%} & 65.8 \up{0.4\%} & \textbf{70.1} \up{1.4\%} & \textbf{60.1} \up{0.8\%} & \textbf{51.3} \up{1.6\%} \\
\midrule\midrule

Vanilla &  & 48.2 & 15.7 & 29.0 & 64.2 & 55.6 & 50.2 & 44.1 \\
Multimodal COT &  & 47.3 & 14.3 & 28.5 & 63.8 & 54.4 & 48.5 & 42.9 \\
CCOT & & 48.0 & 15.6 & 30.2 & 64.0 & 55.5 & 49.3 & 44.5 \\
ICoT &  & 49.8 & 16.0 & 30.6 & 64.7 & 55.9 & 49.6 & 45.0 \\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-5}{*}[1pt]{\rotatebox{90}{\parbox{2.5cm}{\centering \fontsize{11pt}{13pt}\selectfont Qwen2.5 \\ VL 3B}}}
 & \textbf{51.0} \up{2.80\%} & \textbf{17.7} \up{2.74\%} & \textbf{33.3} \up{4.3\%} & \textbf{64.7} \up{0.5\%} & \textbf{56.8} \up{1.26\%} & \textbf{51.2} \up{1.00\%} & \textbf{46.9} \up{2.8\%}\\
\midrule\midrule

Vanilla &  & 61.1 & 23.5 & 41.5 & 62.0 & 68.3 & 58.9 & 50.6 \\\
Multimodal COT &  & 59.6 & 23.1 & 40.6 & 62.8  & 67.2 & 57.1 & 48.2  \\
CCOT &  & 60.5  & 24.8  & 41.8  & 64.6 & 68.0 & 59.0 & 49.4\\
ICoT &  & 61.4 & 25.0 & 42.3 & 65.9 & 68.3 & 58.2 & 50.6 \\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-4}{*}[1pt]{\rotatebox{90}{\parbox{1.0cm}{\centering \fontsize{11pt}{13pt}\selectfont VLAA \\ Thinking 7B}}}
 & \textbf{62.9} \up{1.80\%} & \textbf{27.6} \up{4.10\%} & \textbf{43.9} \up{2.41\%} & \textbf{67.9} \up{5.94\%} & \textbf{69.4} \up{1.1\%} & \textbf{59.2} \up{0.3\%} & \textbf{51.98} \up{1.38\%} \\
\midrule\midrule

Vanilla &  & 51.2 & 18.7 & 40.7 & 62.1 & 67.0 & 52.1 & 50.9 \\
Multimodal COT &  & 52.5 & 18.9 & 39.6 & 62.5 & 68.0 &  51.6 & 51.7 \\
CCOT &  & 53.4 & 20.3 & 40.8 & 63.0 & 68.9 & 53.5 & 52.8 \\
ICoT &  & 55.6  & 21.5 & 41.7 & 63.8 & 69.6 & 54.0 & 54.4 \\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-4}{*}[1pt]{\rotatebox{90}{\parbox{1.2cm}{\centering \fontsize{11pt}{11pt}\selectfont \quad R1 \\ OneVision \quad \quad 7B}}}
 & \textbf{58.0} \up{6.81\%} & \textbf{23.3} \up{4.56\%} & \textbf{42.9} \up{2.21\%} & \textbf{64.1} \up{2.09\%} & \textbf{71.9} \up{4.93\%} & \textbf{56.2} \up{4.14\%} & \textbf{55.4} \up{4.52\%}\\
\midrule\midrule

Vanilla &  & 66.0 & 32.9 & 66.2 & 73.2 & 71.9 & 68.1 & 54.1 \\
Multimodal COT &  & 64.8 & 32.8 & 65.1 & 73.0 & 69.6 & 66.9  &  53.2 \\
CCOT &   & 66.5 & 33.3 & 65.5 & 73.5 & 70.3 & 68.8 & 54.4 \\
ICoT &  & 66.2 & 34.9 & 66.8 & 74.5 & 71.8 & 69.3 & 55.8 \\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-5}{*}[1pt]{\rotatebox{90}{\parbox{2.5cm}{\centering \fontsize{11pt}{13pt}\selectfont Qwen3 \\ VL 8B}}}
 & \textbf{66.9} \up{0.9\%} & \textbf{36.2} \up{3.34\%}& \textbf{67.7} \up{1.51\%} & \textbf{74.6} \up{1.48\%} & \textbf{72.8} \up{0.97\%}& \textbf{70.0} \up{1.91\%} & \textbf{55.6} \up{1.48\%} \\
\midrule\midrule

Vanilla &  & 64.7 & 24.2 & 65.4 & 71.6 & 71.3 & 57.4 & 52.4 \\
Multimodal COT &  & 62.3 & 24.8 & 63.9 & 70.0 & 69.6 & 57.7 & 53.0  \\
CCOT &  & 64.5 &  26.6 & 64.8 & 71.5 & 71.2 & 58.8 & 52.9 \\
ICoT &  & 64.5 & 27.5 & 65.0 & 72.2 & 72.5 & 59.3 & 53.7 \\
\rowcolor{lightblue}
\textbf{\textit{+DMLR (Ours)}} &
\multirow[c]{-5}{*}[1pt]{\rotatebox{90}{\parbox{2.5cm}{\centering \fontsize{11pt}{13pt}\selectfont Qwen3 \\ VL 4B}}}
 & \textbf{65.6} \up{0.93\%} & \textbf{29.4} \up{5.20\%}  & \textbf{65.9} \up{0.5\%} & \textbf{72.7} \up{1.12\%} & \textbf{72.3} \up{0.98\%}& \textbf{60.3} \up{2.88\%} & \textbf{54.9} \up{2.48\%} \\
\bottomrule[1.5pt]
\end{tabular}
}
\vspace{-0.5em}
\label{tab:baseline}
\end{table*}
